LAVA: Label-efficient Visual Learning and Adaptation

We present LAVA, a simple yet effective method for multi-domain visual transfer learning with limited data. LAVA builds on a few recent innovations to enable adapting to partially labelled datasets with class and domain shifts. First, LAVA learns self-supervised visual representations on the source dataset and ground them using class label semantics to overcome transfer collapse problems associated with supervised pretraining. Secondly, LAVA maximises the gains from unlabelled target data via a novel method which uses multi-crop augmentations to obtain highly robust pseudo-labels. By combining these ingredients, LAVA achieves a new state-of-the-art on ImageNet semi-supervised protocol, as well as on 7 out of 10 datasets in multi-domain few-shot learning on the Meta-dataset. Code and models are made available.

==> tables/ablation_losses.tex <==
\begin{table}[]
\centering
\vspace{-2mm}
\scalebox{0.85}{
\begin{tabular}{cccccc}
\toprule[.2em]
% \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textbf{Clipart 690} & \textbf{Clipart 1380} \\   \cline{5-6} 
\multicolumn{1}{l}{$\Lcal_{vl}$} & \multicolumn{1}{l}{$\Lcal_{kc}$} & \multicolumn{1}{l}{$\Lcal_{pl}$} & \multicolumn{1}{l}{} & \textbf{Clipart 690} & \textbf{Clipart 1380} \\ \midrule[0.15em]
$\checkmark$ & $\checkmark$ & $\checkmark$ &  & 48.58 & 58.65 \\
$\checkmark$ & - & $\checkmark$ &  & 48.89 & 55.98 \\
- & $\checkmark$ & $\checkmark$ &  & 47.35 & 57.48 \\
$\checkmark$ & $\checkmark$ & - &  & 44.4 & 43.88 \\
$\checkmark$ & - & - &  & 45.13 & 43.78 \\
- & $\checkmark$ & - &  & 43.17 & 48.79 \\ \bottomrule[0.15em]
\end{tabular}%
}
\vspace{-3mm}
\caption{Results when training our method with different loss settings on {\em Clipart} dataset with 2 and 4 images per class.\vspace{-4mm}}
\label{tab:loss_ablation}
\end{table}









% \begin{table}[h!]
% \centering
% \tiny
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{ccccc}
% \hline
% $\Lcal_{vl}$ & $\Lcal_{kc}$ & $\Lcal_{pl}$ &  & Accuracy \\ \cline{1-3} \cline{5-5} 
% $\checkmark$ & $\checkmark$ & $\checkmark$ &  & 67.93    \\
% $\checkmark$ & -            & -            &  & 66.76    \\
% -            & $\checkmark$ & -            &  & 57.25    \\
% -            & $\checkmark$ & $\checkmark$ &  & 60.12    \\
% $\checkmark$ & $\checkmark$ & -            &  & 62.07    \\ \hline
% \end{tabular}%
% }
% \caption{Average accuracy reported over 100 few-shot episodes of the MSCOCO dataset with different loss settings during fine-tuning.}
% \label{tab:loss_ablation}
% \end{table}

==> tables/cross_domain.tex <==
\begin{table}[]
\centering
\vspace{-2mm}
\scalebox{0.65}{%
\begin{tabular}{lllllll}
\toprule[0.2em]
                                & Clipart & Sketch & Infograph & Quickdraw & Real  & Painting \\ \midrule[0.15em]
Supervised                      & 57.07   & 48.7   & 29.39     & 38.45     & 78.74 & 61.27    \\
Self-supervised        & 52.41   & 46.18  & 29.70     & 36.57     & 79.15 & 64.69    \\ \midrule[0.15em]
\rowcolor{_fbteal3}
\putouralg                            & 58.38   & 50.06  & 31.56     & 40.82     & 79.01 & 63.86    \\ \bottomrule[0.15em]
\end{tabular}%
}
\vspace{-2mm}
\caption{K-NN accuracy on validation sets of DomainNet.\vspace{-4mm}}
\label{tab:x_domain_transfer}
\end{table}

==> tables/init_study.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}



% \begin{table}[]
% \centering
% %\resizebox{\textwidth}{!}{%
\scalebox{0.7}{%
\begin{tabular}{llcclcclcc}
\toprule[0.15em]
 &  & \multicolumn{2}{c}{\textbf{Real}} &  & \multicolumn{2}{c}{\textbf{Clipart}} &  & \multicolumn{2}{c}{\textbf{Quickdraw}} \\ \cline{3-4} \cline{6-10} 
 &  & 2-shot & 8-shot &  & 2-shot & 8-shot &  & 2-shot & 8-shot \\ \hline
Fully-supervised &  & 73.74 & 76.55 &  & 71.87 & 72.75 &  & 61.22 & 67.23 \\ \midrule[0.1em]
\multicolumn{9}{l}{\itshape Initialisation:}\\[1mm]
Sup. \ \ \ (ImNet)$^*$ &  & 54.92 & 64.81 &  & 22.49 & 35.39 &  & 10.68 & 18.78 \\
DINO (ImNet) &  & 46.17 & 59.42 &  & 15.19 & 26.97 &  & 8.98 & 16.81 \\
DINO (Target)$^{**}$ &  & 50.45 & 62.54 &  & 40.35 & 55.03 &  & 30.05 & 43.64 \\ \midrule[0.1em]
\multicolumn{9}{l}{\itshape Fine-tuning from  *:}\\[1mm]
Linear Probing &  & 49.03 & 64.89 &  & 21.5 & 36 &  & 6.08 & 13.9 \\
% DINO AUX &  & 65.58 & 75.41 &  & 36.11 & 61.98 &  & 31.15 & 45.65 \\
MeanTeacher++ &  & 54.26 & 70.60 &  & 34.58 & 60.22 &  & 16.38 & 35.75 \\
\rowcolor{_fbteal3}
\putouralg &  & 57.47 & \textbf{75.41} &  & 38.45 & 64.74 &  & 32.61 & 48.44 \\ \midrule[0.1em]
\multicolumn{9}{l}{\itshape Fine-tuning from  **:}\\[1mm]
Linear Probing &  & 49.68 & 64.42 &  & 38.86 & 56.6 &  & 28.73 & 47.5 \\
% DINO AUX &  & 58.64 & 72.14 &  & 45.52 & 61.47 &  & 32.84 & 51.86 \\
MeanTeacher++ &  & 51.44 & 68.77 &  & 46.02 & 63.09 &  & 29.78 & 47.11 \\
\rowcolor{_fbteal3}
\putouralg &  & \textbf{58.79} & 72.19 &  & \textbf{48.65} & \textbf{65.08} &  & \textbf {36.66} & \textbf{54.91} \\ \bottomrule[0.15em]
\end{tabular}%
}
% \caption{}
% \label{tab:init_study}
% \end{table}

==> tables/semi_sup_results_imagenet.tex <==
% \begin{table}[b]
%     \footnotesize
%     \centering
%     \vspace{-2mm}
%     {\small
    \scalebox{0.8}{
    \begin{tabular}{l r c c c}
        % & & & \multicolumn{2}{c}{\small Top 1}\\
        \small Method & \small Arch. & \small Epochs & \small 1\% & \small 10\% \\\toprule [0.15em]
        \multicolumn{4}{l}{\footnotesize\itshape Different Architecture:}\\[1mm]
        FixMatch~\cite{sohn2020fixmatch} & RN50 & 300 & -- & 71.5 \\
        MPL~\cite{pham2021meta} & RN50 & 800 & -- & 73.9 \\
        SwAV~\cite{caron2020unsupervised} & RN50 & 800 & 53.9 & 70.2 \\
        SimCLRv2++ ~\cite{chen2020big} & RN50 & 1200 & 60.0 & 70.5 \\\midrule[0.15em]
        \multicolumn{4}{l}{\footnotesize\itshape Same Architecture:}\\[1mm]
        DINO-NN~\cite{caron2021emerging} & ViT-S & 300 & 61.3 & 69.1 \\
        DINO~\cite{caron2021emerging} & ViT-S & 350 & 64.5 & 72.2 \\
        \putalg-\textsc{nn}~\cite{assran2021semisupervised} & ViT-S &  300 &  63.5 &  72.3 \\
        \putalg~\cite{assran2021semisupervised} & VIT-S &  300 &  68.9 &  75.2 \\
        \midrule[0.15em]
        \rowcolor{_fbteal3}
        \putouralg-\textsc{nn} & ViT-S & 300 & \bf 67.2 & \bf 73.3 \\
        \rowcolor{_fbteal3}
        \putouralg & ViT-S & 350 & \bf 69.3 & \bf 76.4 \\
        \bottomrule[0.15em]
    \end{tabular}}
%     }
%     \vspace{-2mm}
%     \caption{\small{Comparison to SSL baselines on ImageNet when using 1\% and 10\% of the labels. We report the baselines top-1 accuracy appearing in \putalg~\cite{assran2021semisupervised}, obtained using two size-comparable architectures: RN50 and ViT-S. A suffix of \textsc{nn} denotes the accuracy obtained when performing K-NN classification directly using the pretrained representations.}} %, 
%     \label{table:imagenet_results}
% \end{table}


==> tables/semi_sup_results_imagenet_full.tex <==
\begin{table}[b]
    \footnotesize
    \centering
    \vspace{-2mm}
    {\small
    \begin{tabular}{l r c c c}
        % & & & \multicolumn{2}{c}{\small Top 1}\\
        \small Method & \small Arch. & \small Epochs & \small 1\% & \small 10\% \\\toprule [0.15em]
        \multicolumn{4}{l}{\footnotesize\itshape Pseudo-labelling and Consistency methods:}\\[1mm]
        UDA~\cite{xie2019unsupervised} & RN50 & 800 & -- & 68.1 \\
        FixMatch~\cite{sohn2020fixmatch} & RN50 & 300 & -- & 71.5 \\
        MPL~\cite{pham2021meta} & RN50 & 800 & -- & 73.9 \\\midrule[0.15em]
        \multicolumn{4}{l}{\footnotesize\itshape Representation learning methods:}\\[1mm]
        BYOL~\cite{grill2020bootstrap} & RN50 & 1000 & 53.2 & 68.8 \\
        SwAV~\cite{caron2020unsupervised} & RN50 & 800 & 53.9 & 70.2 \\
        SwAV+CT~\cite{assran2020recovering} & RN50 & 400 & -- & 70.8 \\
        SimCLRv2~\cite{chen2020big} & RN50 & 800 & 57.9 & 68.4 \\
        SimCLRv2++ ~\cite{chen2020big} & RN50 & 1200 & 60.0 & 70.5 \\
        DINO-NN~\cite{caron2021emerging} & ViT-S & 300 & 61.3 & 69.1 \\
        DINO~\cite{caron2021emerging} & ViT-S & 350 & 64.5 & 72.2 \\
        \putalg-\textsc{nn}~\cite{assran2021semisupervised} & RN50 &  300 &  64.2 &  73.1 \\
        \putalg-\textsc{nn}~\cite{assran2021semisupervised} & ViT-S &  300 &  - &  72.3 \\
        \putalg~\cite{assran2021semisupervised} & RN50 &  300 &  66.5 &  75.5 \\
        \midrule[0.15em]
        \multicolumn{4}{l}{\footnotesize\itshape Our method}\\[1mm]
        \rowcolor{_fbteal3}
        \putouralg-\textsc{nn} & ViT-S & 300 & \bf 67.2 & \bf 73.3 \\
        \rowcolor{_fbteal3}
        \putouralg & ViT-S & 350 & \bf 69.3 & \bf 76.4 \\
        \bottomrule[0.15em]
    \end{tabular}}
    \vspace{-2mm}
    \caption{\small{Comparison to baselines and SOTA on ImageNet dataset when using 1\% and 10\% of the labels. We report the baselines top-1 accuracy appearing in \putalg~\cite{assran2021semisupervised}, obtained using two size-comparable architectures: RN50 and ViT-S. A suffix of \textsc{nn} denotes the accuracy obtained when performing K-NN classification directly using the pretrained representations.}} %, 
    \label{table:imagenet_results}
\end{table}

% In our method, this is achieved by discarding the three heads and using the $\texttt{[CLS]}$ token representations to perform nearest neighbours.

==> tables/ssl_and_init.tex <==
\begin{table}[t]
\parbox{.4\linewidth}{
\centering
\caption{\small SSL Comparison on ImageNet with 1\% \& 10\% of the labels.}
\label{table:imagenet_results}
% \vspace{-2mm}
\setlength{\tabcolsep}{2pt}
\scalebox{0.70}{
    \begin{tabular}{l r c c c}
        % & & & \multicolumn{2}{c}{\small Top 1}\\
        \small Method & \small Arch. & \small Epochs & \small 1\% & \small 10\% \\\toprule [0.15em]
        \multicolumn{4}{l}{\footnotesize\itshape Different Architecture:}\\[1mm]
        FixMatch~\cite{sohn2020fixmatch} & RN50 & 300 & -- & 71.5 \\
        MPL~\cite{pham2021meta} & RN50 & 800 & -- & 73.9 \\
        SwAV~\cite{caron2020unsupervised} & RN50 & 800 & 53.9 & 70.2 \\
        SimCLRv2++ ~\cite{chen2020big} & RN50 & 1200 & 60.0 & 70.5 \\\midrule[0.15em]
        \multicolumn{4}{l}{\footnotesize\itshape Same Architecture:}\\[1mm]
        DINO-NN~\cite{caron2021emerging} & ViT-S & 300 & 61.3 & 69.1 \\
        DINO~\cite{caron2021emerging} & ViT-S & 350 & 64.5 & 72.2 \\
        \putalg-\textsc{nn}~\cite{assran2021semisupervised} & ViT-S &  300 &  63.5 &  72.3 \\
        \putalg~\cite{assran2021semisupervised} & VIT-S &  300 &  68.9 &  75.2 \\
        \midrule[0.15em]
        \rowcolor{_fbteal3}
        \putouralg-\textsc{nn} & ViT-S & 300 & \bf 67.2 & \bf 73.3 \\
        \rowcolor{_fbteal3}
        \putouralg & ViT-S & 350 & \bf 69.3 & \bf 76.4 \\
        \bottomrule[0.15em]
    \end{tabular}}
}
\hfill
\parbox{.58\linewidth}{
\centering
\caption{\small Cross-domain performance when using different initialisation and different fine-tuning methods. }
\label{table:init_study}
% \vspace{-2mm}
\setlength{\tabcolsep}{2pt}
\scalebox{0.65}{
\begin{tabular}{llcclcclcc}
\toprule[0.15em]
 &  & \multicolumn{2}{c}{\textbf{Real}} &  & \multicolumn{2}{c}{\textbf{Clipart}} &  & \multicolumn{2}{c}{\textbf{Quickdraw}} \\ \cline{3-4} \cline{6-10} 
 &  & 2-shot & 8-shot &  & 2-shot & 8-shot &  & 2-shot & 8-shot \\ \hline
Fully-supervised &  & 73.74 & 76.55 &  & 71.87 & 72.75 &  & 61.22 & 67.23 \\ \midrule[0.1em]
\multicolumn{9}{l}{\itshape Initialisation:}\\[1mm]
Sup. \ \ \ (ImNet)$^*$ &  & 54.92 & 64.81 &  & 22.49 & 35.39 &  & 10.68 & 18.78 \\
DINO (ImNet) &  & 46.17 & 59.42 &  & 15.19 & 26.97 &  & 8.98 & 16.81 \\
DINO (Target)$^{**}$ &  & 50.45 & 62.54 &  & 40.35 & 55.03 &  & 30.05 & 43.64 \\ \midrule[0.1em]
\multicolumn{9}{l}{\itshape Fine-tuning from  *:}\\[1mm]
Linear Probing &  & 49.03 & 64.89 &  & 21.5 & 36 &  & 6.08 & 13.9 \\
% DINO AUX &  & 65.58 & 75.41 &  & 36.11 & 61.98 &  & 31.15 & 45.65 \\
MeanTeacher++ &  & 54.26 & 70.60 &  & 34.58 & 60.22 &  & 16.38 & 35.75 \\
\rowcolor{_fbteal3}
\putouralg &  & 57.47 & \bf 75.41 &  & 38.45 & 64.74 &  & 32.61 & 48.44 \\ \midrule[0.1em]
\multicolumn{9}{l}{\itshape Fine-tuning from  **:}\\[1mm]
Linear Probing &  & 49.68 & 64.42 &  & 38.86 &  56.6 &  & 28.73 & 47.5 \\
% DINO AUX &  & 58.64 & 72.14 &  & 45.52 & 61.47 &  & 32.84 & 51.86 \\
MeanTeacher++ &  & 51.44 & 68.77 &  & 46.02 & 63.09 &  & 29.78 & 47.11 \\
\rowcolor{_fbteal3}
\putouralg &  & \bf 58.79 & 72.19 &  & \bf 48.65 & \bf 65.08 &  & \bf 36.66 & \bf 54.91 \\ \bottomrule[0.15em]
\end{tabular}}
}
\vspace*{-1.5em}
\end{table} 
